Sym-NCO: Leveraging Symmetricity for Neural Combinatorial Optimization

Deep reinforcement learning (DRL)-based combinatorial optimization (CO) methods (i.e., DRL-NCO) have shown significant merit over the conventional CO solvers as DRL-NCO is capable of learning CO solvers less relying on problem-specific expert domain knowledge (heuristic method) and supervised labeled data (supervised learning method). This paper presents a novel training scheme, Sym-NCO, which is a regularizer-based training scheme that leverages universal symmetricities in various CO problems and solutions. Leveraging symmetricities such as rotational and reflectional invariance can greatly improve the generalization capability of DRL-NCO because it allows the learned solver to exploit the commonly shared symmetricities in the same CO problem class. Our experimental results verify that our Sym-NCO greatly improves the performance of DRL-NCO methods in four CO tasks, including the traveling salesman problem (TSP), capacitated vehicle routing problem (CVRP), prize collecting TSP (PCTSP), and orienteering problem (OP), without utilizing problem-specific expert domain knowledge. Remarkably, Sym-NCO outperformed not only the existing DRL-NCO methods but also a competitive conventional solver, the iterative local search (ILS), in PCTSP at 240 faster speed. Our source code is available at https://github.com/alstn12088/Sym-NCO.

==> section/0_abstract.tex <==
Neural combinatorial optimization (NCO) is a new paradigm of problem-solving strategies for complex NP-hard combinatorial optimization problems (COPs) such as traveling salesman problem (TSP) and capacitated vehicle routing problem (CVRP). Among NCOs, deep reinforcement learning (DRL)-based methods have significant merit, which can learn to design solver without supervised labels attained from the verified solver; thus, it can be applied to un-explorered problems where the verified solver does not exist. However, due to the enormous complexity of the combinatorial solution space, DRL exploration is extremely difficult and degrades performance. In this paper, we suggest leveraging two symmetricity in combinatorial optimization Markov decision process (COMDP) to learn the DRL agent effectively. Firstly, the DRL agent learns SR group (i.e., flip and rotation) equivalency, a universal inductive bias for any CO problems defined on euclidean space: coined \textit{problem-symmetricty}. Secondly, DRL agent explorers symmetric action trajectory using the fact that COP has multiple symmetric optimum solutions: \textit{solution-symmetricity}. To learns MDP symmetricities, we devise a minimax game setting to REINFORCE, where each policy tries to overcome other policy from the same symmetric class. Extensive experiments show that our method significantly improved DRL-based NCO methods; in some COPs, our method achieved better performances than highly engineered classical solvers. 

==> section/0_abstract_new.tex <==
% Deep reinforcement learning (DRL)-based combinatorial optimization (CO) methods have significant merit, which can learn to design solver without supervised labels attained from the verified solver; thus, it can be applied to un-explored problems where the verified solver does not exist. However, due to the enormous complexity of the CO Markov decision process (CO-MDP), DRL exploration is extremely difficult and degrades performance. In this paper, we propose a novel DRL method leveraging symmetricity of the CO-MDP to (a) impose inductive bias for generalization capability and (b) produce high-quality multiple near-optimum solutions. We first construct a transformer-based encoder-decoder model, which is promising in the DRL-CO setting. Then we transform input CO problems using random rotation and flip matrix: they are in the same \textit{problem-symmetric} class. We evaluate the cosine similarity of the projected encoded vectors from same \textit{problem-symmetric} class (by the encoder) with projection head (multi-layer perception): \textit{Invariant loss}. Secondly, we evaluate policy performance (i.e., reward) from \textit{problem-symmetric} class, where each solution is generated without a projection head. By removing the projection head, we can obtain a weakly invariant learned encoder for high randomness in the CO setting. Lastly, policy is learned to produce multiple near-optimal solutions in \textit{solution-symmetric} class by varying multiple root nodes in same \textit{problem-symmetric} class. Specifically, we construct a minimax game setting in REINFORCE method for learning policy to produce a competitive solution than other solutions in the same symmetric class: \textit{Symmetric Loss}. Combining the proposed \textit{Invariant loss} (for inductive bias) and \textit{Symmetric Loss} (for multiple solutions) which regularize each other, our method outperforms previous DRL-CO methods having high generalization capability.           
% Deep reinforcement learning (DRL)-based combinatorial optimization (CO) methods have significant merit, which can learn to design solver without supervised labels attained from the verified solver; thus, it can be applied to un-explored problems where the verified solver does not exist. However, due to the enormous complexity of the CO Markov decision process (CO-MDP), DRL exploration is extremely difficult and degrades performance. In this paper, we propose a novel DRL method leveraging the symmetricity of the CO-MDP for efficient exploration. We first construct a transformer-based encoder-decoder model, which is promising in the DRL-CO setting. Then we transform input CO problems using random rotation and flip matrix: they are in the same \textit{problem-symmetric} class. We evaluate the cosine similarity of the projected encoded vectors from same \textit{problem-symmetric} class (by the encoder) with projection head (multi-layer perception): \textit{Invariant loss}. Secondly, we evaluate policy performance (i.e., reward) from \textit{problem-symmetric} class, where each solution is generated without a projection head. By removing the projection head, we can obtain a weakly invariant learned encoder for high randomness in the CO setting. Lastly, policy is learned to produce multiple near-optimal solutions in \textit{solution-symmetric} class by varying multiple root nodes in same \textit{problem-symmetric} class. Specifically, we construct a minimax game setting in REINFORCE method for learning policy to produce a competitive solution than other solutions in the same symmetric class: \textit{Symmetric Loss}. Combining the proposed \textit{Invariant loss} (for inductive bias) and \textit{Symmetric Loss} (for multiple solutions) which regularize each other, our method outperforms previous DRL-CO methods having high generalization capability. 


Deep reinforcement learning (DRL)-based combinatorial optimization (CO) methods (i.e., DRL-NCO) have significant merit over the conventional CO solvers. DRL-NCO learns CO solvers without supervised labels attained from the verified solver; thus, it can be applied to general CO problems where solvers are not applicable. However, despite its general applicability, many DRL-NCO methods employ problem-specific approaches to derive powerful solvers, possibly limiting the applicability of DRL-NCO for general CO problems. 
% We believe the pursuit of problem-agnosticism in DRL-NCO methods enhances the applicability of DRL-NCO for more general CO problems. 
This paper proposes the DRL-NCO training method that leverages common symmetricities structured in CO problems to improve the performance of DRL-NCO methods. First, we identify the universal symmetricity structure equipped in CO problems. We then propose \ourmethod{}, a regularizer-based training scheme that leveraged the identified symmmetricities that can be applied to various DRL-NCO methods. Our experimental results verify that our method increases the performance of DRL-NCO methods in four CO	 tasks, including traveling salesman problem (TSP), capacitated vehicle routing problem (CVRP), prize collecting TSP (PCTSP), and orienteering problem (OP), without employing problem-specific techniques.

% A slightly modified VER.
% Deep reinforcement learning (DRL)-based combinatorial optimization (CO) methods have significant merit as compared to supervised learning-based approaches as it is trained without the employment of verifies solvers for CO. Thus, they are applicable to solve ``un-explored" CO problems where the verified solver does not exist. However, due to the innate complexity of the CO Markov decision process (CO-MDP), DRL-NCO methods struggle to learn high-performance solvers for general CO tasks. In this paper, we suggest to leverage the symmetricity of CO-MDP to increase DRL-NCO performances and sample efficiency. Firstly, based on the fact that rotation and flip do not change solution optimality of the CO-MDP, we propose a efficient learning techniques to impose those inductive bias to DRL model: problem-symmetricity. Secondly, DRL model is learned to produce multiple (near) optimal solutions if the task contains multiple optimal solutions set: solution-symmetricity. Proposed novel DRL method is verified on multiple representative DRL-NCO models such as pointer network (PN), attention model (AM) and policy optimization and multiple optima (POMO) to show our method is model-agnostic DRL method for CO-MDP. In extensive experimental results show that our method can increase performance of existing DRL-NCO models in four CO tasks: travelling salesman problem (TSP), capacitated vehicle routing problem (CVRP), prize collecting TSP (PCTSP) and orienteering problem (OP). 

==> section/1_intro_jy.tex <==
Combinatorial optimization problems (COPs) are mathematical optimizations on discrete space that carry numerous valuable applications, including vehicle routing problems (VRPs) \cite{cvrp,transportation}, drug discovery \cite{ahn2020guiding,ahn2021spanning}, and semi-conductor chip design \cite{placement1,placement2,liao2020attention}. However, solving COP optimally is difficult as COPs are NP-hard. Therefore, computing satisfactory solutions within an endurable run-time becomes essential from a practical point of view.

% Conventionally, COPs are solved via integer program (IP) solvers and hand-crafted (Meta) heuristics. However, recent advances in computing infrastructures and deep learning conceive a field of neural combinatorial optimization (NCO), a deep learning-based COP solving strategy. Among the NCO approaches, NCO approaches trained by deep reinforcement learning (i.e., DRL-NCO) are specifically favored over conventional approaches due to their applicability to various COPs, trainability without relying on any COP solvers, and their qualified solutions with shorter run times.

Conventionally, COPs are solved via integer program (IP) solvers and hand-crafted (meta) heuristics. Recent advances in computing infrastructures and deep learning conceive a field of neural combinatorial optimization (NCO), a deep learning-based COP solving strategy. Depending on the training method, NCO methods are generally classified into supervised learning \cite{pointer,joshi2020learning,kool_dp,fu2020generalize,hottung2020learning} and reinforcement learning (RL) based approaches. Depending on the solution generation scheme, NCO methods are also classified into improvement \cite{drl-2opt, wu2020learning, NLNS, chen2019learning, mis, kim2021learning, ma2021learning} and construction heuristics \cite{bello2017neural,kool2018attention,Nazari,kwon2020pomo,park2021learning,xin2021multi, park2021schedulenet} \textcolor{red}{which can support orthogonal each other}. Among the NCO approaches, the construction heuristics that are trained by deep RL (i.e., DRL-NCO) are favored over conventional approaches due to their applicability to various COPs, trainability without relying on any COP solvers, and tractability to generate qualified solutions \cite{kool2018attention}. 

% Therefore, the constructive DRL-NCO heuristic is applicable practical domains such as hardware design \cite{liao2020attention}, and molecular design \cite{ahn2021spanning}. 

% Remark that the construction heuristics have high applicability as the problem-specific constrains are easily reflected during solution constructions.  Therefore, the construction heuristic is beneficial to applied practical domain such as hardware design \cite{liao2020attention} and molecular design \cite{ahn2021spanning}. 
Despite the strength and empirical successes of DRL-NCO, the performance gap between the problem-specific state-of-the-art (SOTA) meta-heuristics and DRL-NCO still exist. The DRL-NCO methods close the gaps by employing problem-specific design choices that exploit the problem-specific structures. However, it is generally difficult to identify the problem-specific structures and the method to incorporate such structures into the DRL-NCO methods.

% as it is generally difficult to identify the problem-specific s

% In other words, DRL-NCO loses its problem agnosticism. We believe the problem agnosticism requires to be restored to pursue DRL-NCO as the general COP solving strategy.

In this study, we propose the Symmetric Neural Combinatorial Optimization (\ourmethod{}), a regularizion-based training method that leverages symmetricities \textit{commonly} found in COP, to increase performance of DRL-NCO methods. To this end, we first identify the symmetricities from various COPs, and then device regularizers that can effectively impose the identified symmetricities into the DRL-NCO methods using on the encoder-decoder architecture. The proposed regularizer can be employed to the various COPs because it considers the symmetric structures that are commonly found in COPs.

% In this study, we focus on a training method to revive the problem agnosticism in DRL-NCO by leveraging symmetricity. To be specific, we identify commonly found symmetric structures from COPs (i.e., problem agnostic) and a regularizer-based training method to leverage the symmtericities. It is noteworthy that the regularizer-based training scheme is applicable various DRL-NCO methods. We coin our symmetricity leveraged DRL-NCO training scheme as \ourmethod{}. 
% We expect the acknowledgment of the symmetric structures derives a more generalizable DRL-NCO formula.

\ourmethod{} leverages two types of symmetricities innate in COP that is defined on the Euclidean graph. The first symmetry is the problem symmetry derived from the fact that the rotated graph must exhibit the same optimal solution as the original graph as shown in \cref{figure:problem_sym}. The second symmetry is the solution symmetry that indicates that the permutations of a solution have identical (optimal) costs. For example, the solution to the traveling salesmen problem (TSP) satisfies the solution symmetricity (See \cref{figure:sol_sym}). \ourmethod{} \textit{softly} imposes the identified symmetricities in the form of a regularizer during training. Thus, \ourmethod{} is architecture agnostic.

We experimentally validate \ourmethod{} by applying it into various DRL-NCO methods with their original target problems and observing their performances without employing any problem-specific techniques. By leveraging the symmetricities of COPs, \ourmethod{} can attain the following advantages:
\begin{itemize}[leftmargin=0.5cm]
\vspace{-0.25cm}
    \item \textbf{High performances.} \ourmethod{} achieves near-optimal performance in various tasks (less than 1\%) with extremely high speed (few seconds to solve 10000 instances). Moreover, \ourmethod{} surpasses the competitive PCTSP solver, ILS \cite{kool2018attention}, with 240$\times$ faster speed. 
    \item \textbf{Problem agnosticism.} \ourmethod{} does not employ problem-specific heuristics to solve various COPs. As its empirical evidence, \ourmethod{} is verified to be able to solve TSP, capacitated vehicle routing problem (CVRP), prize collecting TSP (PCTSP), and orienteering problem (OP).
    \item \textbf{Architecture agnosticism.} \ourmethod{} can impose the symmetricities to any encoder-decoder style models using a simple learning scheme. It successfully improved the performance of the various existing DRL-NCO, such as PointerNet \cite{pointer, bello2017neural}, AM \cite{kool2018attention} and POMO \cite{kwon2020pomo}. 
\end{itemize}



==> section/1_intro_new.tex <==
% CO -> DRL-NCO
\textcolor{red}{Combinatorial optimization problems (COP) blah blah (an opening air sentence for explaining CO)}. Conventionally, COPs are solved via exact methods or (meta) heuristics. For many well-known COPs, the conventional methods often provide satisfactory solutions within a durable runtime. Although, the conventional methods can solve the well-known COPs, it has a limiting factor which prevents them to be used in real-world applications where possibly require to handle new types of COPs. That is, they requires extensive amount of human-labor intensive developments to be used in new types of COPs. In recent years, neural combinatorial optimization (NCO), especially the one trained via deep reinforcement learning (RL) formalism (i.e., DRL-NCO), opens a new breakthrough, which automates such development process by learning the solver from the simulations of NCOs. This means that DRL-NCO
can design high-quality solvers for COP that are not yet explored (e.g., A, B, C , and \ndref). Moreover, DRL-NCO posits further practical values such as accelerated computing via GPU parallelization (polynomial time complexity) and near optimal performances backed by the empirical evidences \ndref.

% The technical difficulties of DRL-NCO
With the advances of representation learning capability of DRL methods, the state-of-the-art DRL-NCO solvers \ndref has shown outstanding results. However, training RL agent for solving COP is still known for notoriously difficult (e.g., POMO requires months of training). We conjecture such phenomena is originated from the properties of NCO including \textit{(1)} NCO solvers must well generalize over COPs, unlike the majority of RL tasks that aims to solve one MDP, and \textit{(2)} the equivalency of (optimal) solutions with respect to the action orders. We view those hardships can be understood in a form of innate symmetries in COP as visualized in \textcolor{red}{Fig.X}.

% 
% This paper suggest a method that leverages the symmetries in COP to bring efficient and effective training of DRL-NCO. We overcomes the premonitions limitations by guiding DRL-NCO methods 

% METHOD and Contribution
\textbf{Contribution.} This paper extends the AM-POMO scheme by leveraging the symmetricity of COMDP, making it possible to apply in general COPs (defined in Euclidean space). There are two general symmetricity in COMDP: \textit{problem-symmetricity} and \textit{solution-symmetricity}. For the \textit{problem-symmetricity}, every COPs on Euclidean space has equivalence over SR group action (i.e., rotation and flip): i.e., optimal value does not change in problem rotation and flip. The \textit{problem-symmetricity} is universal property for COPs. 

For the \textit{solution-symmetricity}, some problems have several multiple optimal solutions (TSP, CVRP), some problems have few (Prize collecting TSP: PCTSP), or possibly only one optimal solution. The POMO is a special case to tackle multiple-optima solution sets. In fact, the \textit{solution-symmetricity} must be adaptive founded.   

Because \textit{problem-symmetricity} is universal, it can be leveraged to avoid local-optimum issues using the \textit{shared baseline} scheme of POMO. To be specific, rotation COP must contain the same optimal solutions as the original COP; we can impose a minimax game between two policies from the same \textit{problem-symmetricity} class to overcome each other. Their minimax game leads to the \textit{Nash Equivalence}, in near-optimal solution, having high resistance to fall in bad local optima.

To find \textit{solution-symmetricity} adaptive, we devise multiple sampled solutions in COPs in \textit{problem-symmetricity} and also use it as \textit{shared baseline}: i.e. minimax game. Therefore, (a) each solution in single COPs try to overcome each other and (b) each solution in \textit{problem-symmetricity} class try to overcome each other. Our \textit{joint shared baseline} scheme effectively impose adaptive randomness, can effectively replace POMO's infinite entropy approach.

% A summary of the experimental results.

==> section/1_introduction.tex <==
% CO -> DRL-NCO
Neural combinatorial optimization (NCO), a deep learning-based problem-solving strategy for combinatorial optimization problems (COPs), is drawing considerable attention for two main reasons. Firstly, the NCO method shows possibilities to replace existing classical solvers in COPs using deep neural network (DNN)'s speed (polynomial time complexity with GPU parallelization) and near-optimal performances. DNN can be embedded in classical solving protocols; can improve the speed and performance of classical solvers. However, NCO methods must still be improved to replace classical solvers because it has limitations: generalizability, robustness, and optimality. For example, in traveling salesman problem (TSP), \model{Concorde} gives the optimal solution with a much faster time than state-of-the-art NCO models in every problem size. 

% competitive edge of DRL-NCO
Although NCO shows several limitations on classical COPs such as TSP, NCO has a significant potential value that classical methods do not have. Using deep reinforcement learning (DRL), NCO can automatically design solvers without human experts' direct supervision or classical solver's labeled solutions. This means DRL-based NCOs can design high-quality solvers for COPs tasks that are not yet explored. Because COPs with high industrial value, such as drug design, DNA sequencing, intelligent transportation, hardware design, and chemical synthesis, are not well explored as TSP, DRL-based NCO strategies can be helpful. 


% The technical difficulties of DRL-NCO
However, training the DRL agent for combinatorial optimization Markov decision process (CO-MDP) is extremely hard because (a) the DRL agent learns over problem-distribution (b) even a single problem contains $\mathcal{O}(N!)$ solution trajectories (in TSP). To meet (a), the DRL agent must obtain meta context features over the change of problem distribution which is extremely complex. Also, the DRL agent is easy to stick in local optima because enormous solution spaces give a high chance to attain bias for the DRL agent unless there is strong exploration regularization.

% SOTA models that alleviate the premonitions difficulties
Several works tried to tackle the complexity of CO-MDP. Firstly, Attention Model (\model{AM}) attains remarkable performances over various TSP-variants, using Transformer with context embedding method. AM's context embedding efficiently tackled (a) and applied to several practical applications. Then, Policy Optimization with Multiple Optima (POMO), the DRL algorithm that tackled (b), is proposed. POMO forces entropy of first-action policy to infinite by using symmetric solution space of TSP. Kwon et al. proposed \emph{shared baseline} scheme, which is the average performance of multiple trajectories from the same problem, to devise multiple optima for the DRL agent. The AM trained by the POMO is categorized as state-of-the-art in the DRL-NCO model. 

% the gap
However, AM-POMO has a limitation with extend-ability because POMO's multiple trajectory idea relies on symmetric space of specific COPs such as TSP and capacitated vehicle routing problem (CVRP), which contains (a) circular solution (b) constraint that every node must be visited. These two properties ensure that the entropy of the first-action policy could be infinite because almost every start node contains optimal trajectories. These problem-specific properties highly degrade AM-POMO's task extend-ability, such as:
\begin{itemize}
    \item Non-circular tasks (start and depot are different).
    \item Prize constraint problems (there is an un-visited node).
    \item Stochastic problems (first-action policy must be learned).  
\end{itemize}

% METHOD and Contribution
\textbf{Contribution.} This paper extends the AM-POMO scheme by leveraging the symmetricity of COMDP, making it possible to apply in general COPs (defined in Euclidean space). There are two general symmetricity in COMDP: \textit{problem-symmetricity} and \textit{solution-symmetricity}. For the \textit{problem-symmetricity}, every COPs on Euclidean space has equivalence over SR group action (i.e., rotation and flip): i.e., optimal value does not change in problem rotation and flip. The \textit{problem-symmetricity} is universal property for COPs. 

For the \textit{solution-symmetricity}, some problems have several multiple optimal solutions (TSP, CVRP), some problems have few (Prize collecting TSP: PCTSP), or possibly only one optimal solution. The POMO is a special case to tackle multiple-optima solution sets. In fact, the \textit{solution-symmetricity} must be adaptive founded.   

Because \textit{problem-symmetricity} is universal, it can be leveraged to avoid local-optimum issues using the \textit{shared baseline} scheme of POMO. To be specific, rotation COP must contain the same optimal solutions as the original COP; we can impose a minimax game between two policies from the same \textit{problem-symmetricity} class to overcome each other. Their minimax game leads to the \textit{Nash Equivalence}, in near-optimal solution, having high resistance to fall in bad local optima.

To find \textit{solution-symmetricity} adaptive, we devise multiple sampled solutions in COPs in \textit{problem-symmetricity} and also use it as \textit{shared baseline}: i.e. minimax game. Therefore, (a) each solution in single COPs try to overcome each other and (b) each solution in \textit{problem-symmetricity} class try to overcome each other. Our \textit{joint shared baseline} scheme effectively impose adaptive randomness, can effectively replace POMO's infinite entropy approach.

% A summary of the experimental results.

==> section/2_rel_work.tex <==
%\paragraph{Deep Symmetric Learning} Deep learning leveraging symmetricities of data is a promising method to improve the DNN model's generalization capability and sample efficiency in several domain tasks. Typical deep symmetric learning is self-supervised learning (SSL), which leverages symmetries of data (usually) to train the vision model and language model to increase model generalization capability under limited labeled data. SSL is a method that uses a transformation function such as data augmentation (DA) into input data, making the DNN model figure out the transformation function. The transformation function includes image rotation and sentence permutation, where these functions usually preserve data's invariant characteristics\footnote{Note that in CV and NLP tasks, finding a perfect transformation function that preserves data's invariant characteristics is hard. For example, rotation may hurt data invariant if '6' is rotated to '9'. }: i.e., original data and transformed data are (possibly) symmetric. Because SSL can increase sample efficiency and generalization capability, SSL is also applied to reinforcement learning tasks \cite{srinivas2020curl}.

While the SSL scheme learns symmetiricities using a loss scheme, some researchers focus on imposing data symmetricities by giving hard-constraint to neural network architecture: the equivariant neural network (ENN) scheme. \cite{niu2020permutation} suggested permutation equivariant graph neural network, which gives equivariant output for input permutation-transformed data. \cite{fuchs2020se} proposed an equivariant transformer network for point cloud data, which gives equivariant output for SO(3) group input transformation. Moreover, the equivariant graph neural network (EGNN) \cite{satorras2021n} can produce O(n) group equivariant output. These ENN can reduce the search space of the model dramatically; some research applied to reinforcement learning tasks for sample efficiency \cite{van2020mdp}.  

Our research is deep symmetric learning for combinatorial optimization. We did not give hard-constraint to the neural network but devised an SSL style loss scheme. That is because hard-equivariant constraints to neural networks may hurt the NCO model's diversity. We discuss it with some experimental results in the discussion section.  

\subsection{Neural Combinatorial Optimization} Neural combinatorial optimization (NCO) is a deep learning-based problem-solving strategy for complex problems such as NP-hard routing problems. NCO is categorized as a deep constructive heuristic (DCH) or deep improvement heuristic (DIH). In DCH, the DNN model sequentially constructs part of the solution to complete the set from the empty set. The DCH is beneficial to task expandability because the model can consider rules and constraints in each solution construction step. Moreover, DCH is capable of online settings where additional nodes are imposed in the problem without fully re-optimization. 

In DIH, model iterative improves solution, usually starting from a random feasible solution. The DIH is beneficial for making high-quality solution to compare with DCH when the time budget is sufficient because DIH can iterative improves solution quality. Furthermore, DIH can collaborate with DCH, where DCH gives initial high-quality seeds, then DIH improves to seeds. 

While DCH and DIH are end-to-end deep learning methods, some research blends deep learning and classical method for state-of-the-art performances in specific tasks. These methods give promising performances by accelerating the classical method's speed bottleneck using DNN models' fast inference. However, these hybrid methods inherit low flexibility from the classical method, hard to expand to general practical tasks. 

%\textbf{Practical Applications of NCO.} There are several pieces of research that target high-impact practical tasks, including hardware optimization \cite{liao2020attention,track,kim} and molecular optimization \cite{ahn2020guiding,ahn2021spanning} over the classical CO benchmarks such as TSP and CVRP. Usually, transformer-style deep constructive heuristics are widely used in practical tasks because rule-violating is a critical difficulty in practical tasks such as molecular generation. For example, \cite{ahn2021spanning} proposed transformer-based DCH as a generative model for molecular design, showing each design keeps specific chemical rules. Our method is also a deep constructive heuristic for general-purpose CO, including practical design tasks. Our method (designed for general encoder-decoder NCO) is verified on the attention model (AM), which is a transformer-style constructive heuristic.  


%\textbf{Deep Symmetric Learning in NCO.} There are several symmetrical learning approaches in NCO; the POMO is a representative method. POMO is a DCH model which gives extremely high performances in TSP and CVRP. POMO's neural network architecture is similar to the existing DCH model, AM \cite{kool2018attention}, but gives more efficient performances using a simple scheme: the \textit{shared baseline}. The \textit{shared baseline} is used to produce multiple (near) optimal solutions using solution symmetricities in TSP and CVRP. Because TSP has N symmetric solution having heterogeneous root nodes, POMO set rewards from each trajectory are competing with each other using the \textit{shared baseline}. However, POMO's symmetric learning method is limited to a problem with multiple optimal solution sets such as TSP. Our method is an expansion of POMO, using both problem symmetricity and solution symmetricity to solve general CO-MDP tasks. See the Appendix to see a detailed technical difference between our method and POMO. 

==> section/3_sym_comdp.tex <==
This section provide formulation of neural combinatorial optimization and define symmetricity on the formulation.  


\subsection{Combinatorial Optimization Markov Decision Process (CO-MDP)}

Neural combinatorial optimization (NCO) aims to design DNN solver $P_\theta$ to produce optimal solution from problem $\boldsymbol{x}$ and feature $\boldsymbol{f}$ generated from distribution $\rho$:

\begin{equation}
    {\theta}^*= \argmax \mathbb{E}_{\{\boldsymbol{x},\boldsymbol{f}\}\sim\rho}\mathbb{E}_{\boldsymbol{\pi} \sim P_\theta(\cdot|\{\boldsymbol{x},\boldsymbol{f}\})}R(\boldsymbol{\pi})
\end{equation}

We formulate TSP-style neural combinatorial optimization as Combinatorial optimization Markov decision process (CO-MDP)\footnote{Other task defined of 2D euclidean space can be expressed similarly with TSP-style only with small modification}:

\textbf{Instance distribution.} Instance distribution $\rho$ is probability distribution function (PDF) which samples problem $\boldsymbol{x}$ and problem featrue $\boldsymbol{f}$. Usually, NCO researches set $\rho$ as uniform distribution. 

\textbf{Problem.} Problem $\boldsymbol{x}=\{x_1,...,x_N\}$ is 2D euclidean nodes, indicating location of cities.  

\textbf{Problem Feature.} Problem feature $f$ is node features corresponding problem $s$ such as prize and demand. In TSP, there is no problem feature.  

\textbf{State.} The state $\boldsymbol{s}_t$ contains previous selected nodes $\boldsymbol{a}_{1:t}$ and $\{\boldsymbol{x},\boldsymbol{f}\}$: $\boldsymbol{s}_t = \{\boldsymbol{a}_{1:t}|\{\boldsymbol{x},\boldsymbol{f}\}\}$. Note that initial state is $\{\boldsymbol{x},\boldsymbol{f}\}$ which is random variable of $\rho$ which makes CO-MDP special. 

\textbf{Action.} The action $a_t$ is node selection of un-visited nodes: $a_t \in \{ \{1,...,N\} \setminus \{\boldsymbol{a}_{1:t-1}\} \}$. 

\textbf{Solution.} The solution $\boldsymbol{\pi} = \boldsymbol{s}_{T}$ is terminal state where step $t$ is terminated in $T$.

\textbf{Reward.} The reward is objective of the task. Reward is function of $\boldsymbol{a}_{1:T}$ (solution sequences), $||x_i - x_j||_{i,j \in \{1,...N\}}$ (relative distances) and $\boldsymbol{f}$ (nodes features including prize). In TSP, CVRP and PCTSP reward is negative of tour length. In OP, reward is sum of prize. 

\textbf{Policy.} Policy $p_{\theta}(a_t|\boldsymbol{s}_t)$ produces action $a_t$ from problem $s_t$. The solver is defined as:

$P_{\theta} = \prod_{t=1}^{T} p_{\theta}(a_t|\boldsymbol{s}_t)$.

\subsection{Symmetricities in CO-MDP}
There are several difficulties of solving CO-MDP; one of the difficulty is that initial state is random variable of $\rho$. The solver $P_\theta$ should produce high quality solution from random problem $\boldsymbol{x}$, which requires significant generalization capabilities. 

The generalization capability of DNN solver can be increased when we capture common information of CO-MDP: symmetricity. There are two major symmtricities can be defined. 



\textbf{Solution Symmetry.} Let $\boldsymbol{\Pi} = \{\boldsymbol{\pi^1},...,\boldsymbol{\pi^k}\}$ is solution set where, $R(\boldsymbol{\pi^1}) = ... = R(\boldsymbol{\pi^k})$. Then solution $\boldsymbol{\pi^i}$ and $\boldsymbol{\pi^j}$ is solution symmetric: $\boldsymbol{\pi^i} \sim \boldsymbol{\pi^j}$. 

\textbf{Problem Symmetry.} Problem $\boldsymbol{x}^i$ and $\boldsymbol{x}^j$ are problem symmetric, $\boldsymbol{x}^i \sim \boldsymbol{x}^j$ if they have identical optimal solution set given same problem feature $\boldsymbol{f}$: $P_{\theta^*}(\{\boldsymbol{x}^i,\boldsymbol{f}\}) = P_{\theta^*}(\{\boldsymbol{x}^j,\boldsymbol{f}\}).$ 

We find universal solution symmetry of CO-MDP, using orthogonal matrix; rotation and flip does not change optimal solution set:

\textbf{Theorem 1.} \textit{Any problem $\boldsymbol{x}$  and $Q(\boldsymbol{x})$ in the CO-MDP is problem symmetry: i.e, $\boldsymbol{x} \sim Q(\boldsymbol{x})$ , if $Q$ is orthogonal matrix.} 

\textit{Proof.} See Appendix.


% For all $x_i, x_j \in \boldsymbol{x}$

% $||x_i - x_j|| = (x_i - x_j)^{T}(x_i-x_j) = (x_i-x_j)^{T}Q^{T}Q(x_i-x_j) = (Qx_i - Qx_j)^{T}(Qx_i-Qx_j) = ||Qx_i - Qx_j||$ 

% For any $\boldsymbol{\pi} \in \boldsymbol{\PI^{*}|_{\boldsymbol{x}}}$, 
% $R(a|$






==> section/4_sym_nco.tex <==


This section presents our Symmetric Neural Combinatorial Optimization (Sym-NCO) algorithm. The Sym-NCO is designed to be applied any encoder-decoder style NCO methods including pointer-network, attention model (AM) and policy optimization for multiple optima (POMO) to enhance the use of explained symmetricities in NCO. Our method comprise of three distinctive loss: $\mathcal{L}_{\text{inv}}, \mathcal{L}_{\text{ps}}, \mathcal{L}_{\text{ss}}$.


\subsection{Imposing the Invariant Encoder Representation using $\mathcal{L}_{\text{inv}}$.}

In NCO, encoder architecture map problem $s$ to high dimensional representation $h$. By the Theorem 1, for any orthogonal matrix $Q$, $s \sim Q(s)$. Therefore, we can force to encoder map invariant representation of problem symmetric space. 

These inductive bias may helpful to increase sample efficiency and generalization capability, because they are invariant characteristic for every CO-MDP. However, imposing $Q$ invariant characteristic can also decreases model's diversity, which is crutial for NCO solver (generating multiple near-optimal solution is important). 

To impose $Q$ invariant effectively preserving model's diversity, we applied projection head to representation $h$, similarly with the SimCLR method in image recognition. Specifically, we define invarinat loss:
\begin{equation}
    \mathcal{L}_{\text{inv}} = -sim(g(h|_{s}), g(h|_{Q(s)}))
\end{equation}
Where $g$ is multi-layer perceptron (MLP) projection head and the $sim$ is consine similarity of two vectors. By removing projection head in decoding process, we can preserve diversity of model. 


\subsection{Learning Encoder-decoder to Produce Diverse Near-optimal Solutions using $\mathcal{L}_{\text{ps}}, \mathcal{L}_{\text{ss}}$.}

Producing diverse near-optimal solution is crucial for NCO solver, because we can collect best solution among produced samples. Symmetricity of CO-MDP can be exploited to learn diversity of DNN solver. Using solution symmetricity, we suggest new policy gradient method:
\begin{equation}
    \nabla \mathcal{L}_{\text{ss}} = -E_{\boldsymbol{x} \sim \rho}E_{\boldsymbol{\pi}^1,..,,\boldsymbol{\pi}^K \sim P_{\theta}(\cdot|\boldsymbol{x})} [(R(\boldsymbol{\pi}) - \frac{1}{K}\sum_{i=1}^{K} R(\boldsymbol{\pi}^{i})) \nabla log P_{\theta} ]
\end{equation}
 
%  In TSP, there are at least $N$ optimal solution which has different root node. In this case we can just manually diverse N difference root node as $\boldsymbol{a}_i = i$, as POMO did (i.e. POMO is special case of ours). However, in other problems $P_1$ must be learned to produce root nodes, because solution symmetricity from different root node is not general properties. The (3) gives general expansion of POMO's shared baseline method, where $P_1$ is automatically learn to produce diverse solution which try to overcome other solutions: minimax setting. 

Similarly, we devise another policy gradient loss by using the fact that $\boldsymbol{x} \sim Q(\boldsymbol{x})$ has same optimal solution set:
\begin{equation}
    \nabla \mathcal{L}_{\text{ps}} = -E_{\boldsymbol{x} \sim \rho} E_{\boldsymbol{Q} \sim q}E_{\boldsymbol{\pi}^{11},..,,\boldsymbol{\pi}^{KL} \sim P_{\theta}(\cdot|\boldsymbol{x},\boldsymbol{Q})} [(R(\boldsymbol{\pi}) - \frac{1}{LK}\sum_{j=1}^{L}\sum_{i=1}^{K} R(\boldsymbol{\pi}^{ij}|Q_j(\boldsymbol{x}))) \nabla log P_{\theta} ]
\end{equation}
Where $q$ is random distribution to produce orthogonal matricies $\boldsymbol{Q} = \{Q_1, ...,Q_{L}\}$.  


\subsection{Learning Scheme}

To sum up, NCO models can be learned in Sym-NCO style to minimize following loss:
\begin{equation}
    \mathcal{L}:= \alpha \mathcal{L}_{\text{Inv}} + \beta \mathcal{L}_{\text{ps}} + \gamma \mathcal{L}_{\text{ss}}
\end{equation}
The $\alpha, \beta, \gamma$ is hyperparameters. Note that these hyperparameters are easily tun-able; we only set $\alpha \in \{0.1,0.2\}$, $\beta = 1$, $\gamma = \{0,1\}$.





==> section/4_sym_nco3.tex <==
% \label{sec:sym-nco}

% \begin{figure}[t]
% \centering
% % \includegraphics[width=0.9\textwidth]{figures/figure2.png}
% \includegraphics[width=1.0\textwidth]{figures_new/sym_nco_cropped.pdf}
% \caption{An overview of \ourmethod{}}
% \end{figure}

% This section presents Symmetric Neural Combinatorial Optimization (\ourmethod{}). It is an effective training scheme that leverage the symmetricities of CO-MDP. We explain the details of \ourmethod{} in the context of encoder-decoder style NCO trained with the policy gradient method \cite{pointer, kool2018attention, kwon2020pomo}. \ourmethod{} imposes the symmetricities to $F_\theta$ by minimizing the symmetric loss function defined as follows:
% \begin{align}
%     \mathcal{L_{\text{sym}}}= 
%     \alpha \mathcal{L}_{\text{inv}} + 
%     \psl + 
%     \beta \ssl
% \end{align}
% where $\mathcal{L}_{\text{inv}}$, $\mathcal{L}_{\text{ps}}$, and $\mathcal{L}_{\text{ss}}$ are loss function that imposes invariant representation, problem symmetry, and solution symmetric, respectively. $\alpha, \beta \in [0,1]$ are the weight coefficients. In the following subsections, we explains each loss component in detail.

% \subsection{Imposing invariant problem representation via $\mathcal{L}_{\text{inv}}$.}
% For most NCO methods, the encoder network maps $P=(x,f)$ to high dimensional vector representation $h$. By \cref{thm:rot_sym}, for any orthogonal matrix $Q$, $x \sym Q(x)$. Therefore, it can be reasonable that the encoder maps the rotational symmetric problems into the same hidden representation.

% The rationally invariant $h$ can be attained through the invariant encoder architecture \cite{satorras2021n} or minimizing the discrepancy between $h(x)$ and $h(Q(x))$ \cite{chen2020simple}. 
% However, the approach utilizing invariant encoder architecture limits the use of flexible architecture including Transformer \cite{transformer}. The approach to minimizing the discrepancy can map every $h(x)$ to similar ones. 
% % However, the architecture approach limits the architecture of the encoder to the specific designs (e.g., Transformer \cite{transformer} cannot be used.), and the penalization can deteriorate the diversity of $h$, which is known to be a crucial aspect of NCO solver \cite{kwon2020pomo}. 

% To allow the use of arbitrary encoder network architecture while maintaining the diversity of $h$, we propose to penalize the discrepancy among the projected $h$s inspired by \cite{chen2020simple}. To be specific, we define the invariant representation loss $\mathcal{L}_{\text{inv}}$ as follows:
% \begin{align}
%     \mathcal{L}_{\text{inv}} = -S_\text{cos}\bigg(g\Big(h(x)\Big), g\Big(h\big(Q(x)\big)\Big)\bigg)
% \end{align}
% where $S_\text{cos}(a,b)$ is the cosine similarity between $a$ and $b$, $g(\cdot)$ is the MLP-parameterized projection head. By feeding $h$ to the decoder, we impose the problem symmetricities while maintaining the representation capability of the encoder. We empirically found this soft approach helps to attain stronger solvers as described in \cref{subsec:hard_const}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% JKP edited %%%%%%%%%%%%%%%%%%%%%%%

\label{sec:sym-nco}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\textwidth]{figures_new/sym_nco_cropped.pdf}
\caption{An overview of \ourmethod{}}
\end{figure}

This section presents Symmetric Neural Combinatorial Optimization (\ourmethod{}). It is an effective training scheme that leverage the symmetricities of CO-MDP. We explain the details of \ourmethod{} in the context of encoder-decoder style NCO trained with the policy gradient method \cite{pointer, kool2018attention, kwon2020pomo}. \ourmethod{} imposes the symmetricities to $F_\theta$ by minimizing the symmetric loss function defined as follows:
\begin{align}
    \mathcal{L_{\text{sym}}}= 
    \alpha \mathcal{L}_{\text{inv}} + 
    \psl + 
    \beta \ssl
\end{align}
where $\mathcal{L}_{\text{inv}}$, $\mathcal{L}_{\text{ps}}$, and $\mathcal{L}_{\text{ss}}$ are loss function that imposes invariant representation, problem symmetry, and solution symmetric, respectively. $\alpha, \beta \in [0,1]$ are the weight coefficients. In the following subsections, we explains each loss component in detail.





\subsection{Imposing invariant problem representation via $\mathcal{L}_{\text{inv}}$.}
By \cref{thm:rot_sym}, the original problem $x$ and its transformed problem $Q(x)$ (rotation of the problem) has the same solutions, i.e., $x \sym Q(x)$, for any orthogonal matrix $Q$. We impose this solution symmetricity into the encoder of NCO solvers by using the rotation invariant representation. 


Let's denote $h(x)$ to be the hidden representation (high dimensional vector) of the input problem $x$ and $(h(Q(x))$ the hidden representation of the transformed input problem $x$. To impose rotational invariant representation of the hidden representation $h$, the loss function $\mathcal{L}_{\text{inv}}$ is defined:
\begin{align}
    \mathcal{L}_{\text{inv}} = -S_\text{cos}\bigg(g\Big(h(x)\Big), g\Big(h\big(Q(x)\big)\Big)\bigg)
\end{align}
where $S_\text{cos}(a,b)$ is the cosine similarity between $a$ and $b$. Instead of directly penalizing the difference between $h(x)$ and $(h(Q(x))$, we penalize the difference between their projected representation, $g(h(x))$ and $g((h(Q(x)))$, with  $g(\cdot)$ being the MLP-parameterized projection head. This penalizing scheme allow the use of arbitrary encoder network architecture while maintaining the diversity of $h$ \cite{chen2020simple}. We empirically found this ''soft'' approach helps to attain stronger solvers as described in \cref{subsec:hard_const}.


Note that the rotation invariant $h$ can also be attained through the invariant encoder architecture \cite{satorras2021n}. However, this approach inevitably restricts the flexibility of the encoder architecture, thus preventing the use of flexible architectures, like a Transformer \cite{transformer}. We have empirically validated that our approach is more effective than using the invariant architecture. 





























\subsection{Imposing problem and solution symmetricities via $\psl{}$ and $\mathcal{L}_{\text{ss}}$}

% =============================================================================================

As discussed in \cref{subsec:sym-co-mdp}, CO-MDP contains the problem and solution symmetricities. In this subsection, we explain $\psl$ and $\ssl$ which is used to train $F_\theta$ while respecting the symmetricities. Let us consider an instance of problem $P=(x,f)$ and its solution $\sol(P)$. Then the gradient of the problem symmetricity loss for $\sol(P)$ is defined as:
\begin{align}
    \nabla_\theta \psl(\sol(P)) = -\mathbb{E}_{Q^l \sim \rmQ}
    \bigg[
        \mathbb{E}_{\sol^{l,k} \sim F_\theta(Q^l(P))}
        \Big[
            \big[R(\sol(P))-\frac{1}{LK}\sum_{l=1}^{L}\sum_{k=1}^{K}R(\sol^{l,k})
            \big]\nabla_\theta \log F_\theta(\sol(P))
        \Big]
    \bigg]
\end{align}
where $\rmQ$ is the distribution of random orthogonal matricies, $L$ and $K$ are the number of problem and solution sysmmteric samples, and $\log F_\theta(\sol(P))$ is the log-likelihood of $F_\theta$ to generate $\sol(P)$. Intuitively speaking, If a solver $F_\theta$ minimizes $\psl$ for all $P \in \rho$, then $F_\theta$ is the optimal solver while maintaining the problem symmetricity (\cref{def:pro_sym}, \cref{thm:rot_sym}).

Similarly, we also define the gradient of solution symmetricity loss for $\sol(P)$ is defined as:
\begin{align}
    \nabla_\theta \ssl(\sol(P)) = -\mathbb{E}_{\sol^k \sim F_\theta(P)}
    \big[
    (R(\sol(P))-\frac{1}{K}\sum_{k=1}^{K}R(\sol^k))\nabla \log F_\theta(\sol(P))
    \big]
\end{align}

\ch{In TSP, minimization of $\ssl$ implies $F_\theta$ attains the solution symmetricity (\cref{def:sol_sym}) when we assure $\{\sol^{j}\}_{j=1}^{K}$ choose every cities as their starting nodes. A similar approach is implemented in POMO \cite{kwon2020pomo}. In CVRP, minimization of $\ssl$ may nearly attains solution symmetricity; hence we samples $K$ solutions from $F_\theta(P)$. In PCTSP and OP, the existence of solution symmetricities is not proven. Therefore, we exclude $\ssl$ by setting $\beta$ as 0 and set $K=1$.}

% ==============================================================================================

% As discussed in \cref{subsec:sym-co-mdp}, CO-MDP contains the problem and solution symmetricities. In this subsection, we explain $\psl$ and $\ssl$ used to train $F_\theta$, while respecting the symmetricities by expanding the \textit{shared baseline} scheme \cite{kwon2020pomo}. Let us consider an instance of problem $P=(x,f)$ and its solution $\sol(P)$. Then the gradient of the problem symmetricity loss for $\sol(P)$ is as follows:
% \begin{align}
% \nabla_{\theta} \psl \approx -\frac{1}{LK} \sum_{i=1}^{L}\sum_{j=1}^{K}\left(\left(R\left(\boldsymbol{\pi}^{i,j}\right)-\frac{1}{LK} \sum_{i=1}^{L}\sum_{j=1}^{K} R\left(\boldsymbol{\pi}^{i,j}\right) \right) \nabla_{\theta} \log F_{\theta}\left(\boldsymbol{\pi}^{i,j} \mid P,\boldsymbol{Q}\right)\right)
% \end{align}


% where $\rmQ$ is the distribution of random orthogonal matricies, $L$ and $K$ are the number of problem and solution sysmmteric samples, and $\log F_\theta(\sol(P))$ is the log-likelihood of $F_\theta$ to generate $\sol(P)$. Intuitively speaking, If a solver $F_\theta$ minimizes $\psl$ for all $P \in \rho$, then $F_\theta$ is the optimal solver while maintaining the problem symmetricity (\cref{def:pro_sym}, \cref{thm:rot_sym}).

% Similarly, we also define the gradient of the solution symmetricity loss for $\sol(P)$ is as follows:
% \begin{align}
% \nabla_{\theta} \ssl \approx -\frac{1}{K} \sum_{j=1}^{K}\left(\left(R\left(\boldsymbol{\pi}^{j}\right)-\frac{1}{N} \sum_{j=1}^{K} R\left(\boldsymbol{\pi}^{j}\right) \right) \nabla_{\theta} \log F_{\theta}\left(\boldsymbol{\pi}^{j} \mid P\right)\right)
% \end{align}

% In TSP, minimization of $\ssl$ implies $F_\theta$ attains the solution symmetricity (\cref{def:sol_sym}) when we assure $\{\sol^{j}\}_{j=1}^{K}$ choose every cities as their starting nodes. A similar approach is implemented in POMO \cite{kwon2020pomo}. In CVRP, minimization of $\ssl$ may nearly attains solution symmetricity; hence we samples $K$ solutions from $F_\theta(P)$. In PCTSP and OP, the existence of solution symmetricities is not proven. Therefore, we exclude $\ssl$ by setting $\beta$ as 0 and set $K=1$. 

% ==============================================================================================




















\paragraph{Game theoretical interpretation.} \ch{The \textit{shared baseline} scheme can be interpreted as the \textit{minimax} game. To be simple interpretation, let $K=1$. The advantage of policy gradient loss in $\lps$ is evaluate as substitute of $R(\sol^{i})$ (reward of solution from $P$), and $\frac{1}{L} \sum_{i=1}^{L} R(\sol^{i})$ (rewards of solutions from same problem symmetric class of $\mQ(P)$). Therefore, each policy $p(\pi^{i}|P,Q_i)$ and $p(\pi^{j}|P,Q_j)$ compete each other. We view this process has high resistance to bad local optimum, because if some policy $p(\pi^{i} \vert P, Q_i)$ may find better solution spot than the local optimum, other policies $p(\pi^{i} \vert P, Q_j)$ (may felled in the local optimum) tries to find better spot.}

% \ch{Note that only exploiting problem symmetricities still offers significant performance gain in TSP (which has $N$ solution symmetricities), as shown in Section 4.}    

==> section/5_3_ablation.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[t]{0.32\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{figures/tsp_ablation.png}
         \includegraphics[width=\textwidth]{figures_new/tsp100_epoch_cost.pdf}
         \caption{Cost curves of different loss designs}
         \label{fig:loss_design_cost_plot}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.32\textwidth}
        \centering
        %  \includegraphics[width=\textwidth]{figures/cvrp_ablation.png}
        %  \includegraphics[width=\textwidth]{figures_new/cvrp100_epoch_cost.pdf}
        \includegraphics[width=\textwidth]{figures_new/cos_similarity_inv_loss.pdf}
        \caption{Cosine similarity curves}
        \label{fig:cos_sim_plot}
     \end{subfigure}
        \begin{subfigure}[t]{0.32\textwidth}
        \centering
        %  \includegraphics[width=\textwidth]{figures/similarity.png}
        % \includegraphics[width=\textwidth]{figures_new/cos_similarity_inv_loss.pdf}
        \includegraphics[width=\textwidth]{figures_new/proj_head_ablation.pdf}
        \caption{Projection head ablation results}
        \label{fig:proj_head_plot}
     \end{subfigure}
    \caption{\textbf{Loss design ablation results.} (a) Effect of loss components to the costs, (b) Cosine similarity curves of the models with and with $\mathcal{L}_{\text{inv}}$, (c) Costs of the models with and without $g(\cdot)$.}
\end{figure}







% \ch{This section provides ablation study of proposed loss scheme. As shown in Figure 2, $L_{ss} + L_{ps} + L_{inv}$ scheme gives most efficiency learning curve to compare with $L_{ss} + L_{ps}$ and $L_{ss}$. Note that NCO baseline POMO is algorithm that only used $L_{ss}$. \textcolor{red}{As shown in Fig X, $L_{inv}$ effectively increase consine simliarility in the projection space: i.e., invaraint learning is effectively done)}.} 



% Leveraging symmetricity is a very important idea for specific CO tasks at this time and in further directions. Several studies tried to use symmetricities in CV, NLP, and graph tasks, as we mentioned in section 4. 

% In this work, we devise symmetricities of CO-MDP by using $L_{inv}$, using the SimCLR style projection head scheme. We find that leveraging symmetricity in CO-MDP is hard because RL exploration needs sufficient randomness to provide a near-optimal solution. Giving too hard a constraint may hurt the model's exploration, degrading performances. 

 

==> section/5_ablation.tex <==
\subsection{Ablation Study}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tsp_ablation.png}
         \caption{TSP100}
         \label{TSP100}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cvrp_ablation.png}
         \caption{CVRP100}
         \label{CVRP100}
     \end{subfigure}
        \caption{Ablation study}
      
\end{figure}

\textbf{Ablation Study of Loss Scheme.} This section provides ablation study of proposed loss scheme. As shown in Figure 2, $L_{ss} + L_{ps} + L_{inv}$ scheme gives most efficiency learning curve to compare with $L_{ss} + L_{ps}$ and $L_{ss}$. Note that NCO baseline POMO is algorithm that only used $L_{ss}$. 

\textbf{Sym-NCO Application to Other NCO Models:} See Appendix X.

\textbf{Larger Scale Adaptation Evaluation:} See Appendix X.

\textbf{Ablation Study of Real-world TSP (TSPLIB):} See Appendix X. 

\textbf{Ablation Study of Hyperparameters:} See Appendix X.

==> section/5_experiments.tex <==
This section provides experimental results of the proposed \textit{Sym-NCO} on four COP tasks: TSP, CVRP, PCTSP, and OP. In TSP and CVRP, Sym-NCO is coping with POMO, which is one of the most powerful deep constructive heuristic in TSP and CVRP. 

Note that we also show Sym-NCO can improve other NCO method such as attention model (AM) and pointer newtork (PointerNet) in representative CO methods such as TSP, see Appendix for details. 
In PCTSP and OP, Sym-NCO improves AM method, having most competitive results. Note that in PCTSP and OP there are no POMO application. 

We provide an important disputes in NCO researches with our argument before reporting performance evaluate as below:



\textbf{Problem Scale.} Because several researches shows great results in $N=20,50$, we skip to report results in such a scales; we focus on $N=100$. We realize that there are concerns about scalability of NCO method because there are only fixed scale training-inference verification in past. Recently, several researches tried to tackle scalability issue using \textit{existing NCO models}. For example, \cite{lisicki2020evaluating} suggested \textit{curriculum learning} scheme to improves scale adaptation ability. \cite{hottung2021efficient} suggested a novel transfer learning style active search scheme that improves performances of NCO model on larger scale tasks. Therefore, we can conclude that both (1) providing effective base NCO model is important (2) providing effective scalability scheme for existing NCO model is important, where we focus on (1) issue. However, we also show scalability performance in \textcolor{red}{Appendix X} making collaboration with \textit{Sym-NCO} and \cite{hottung2021efficient}, to verifies potential scalability of our method. 

\textbf{Speed Evaluation.} Speed evaluation is crucial part in COP solvers performances because every solver can achieve an \textit{Optimal} solution if there is infinite time budget. However, evaluating speed in fair is difficult or maybe impossible. Firstly, speed comparison with classical heuristic solver and NCO solver is hard because classical solver is implemented on the \textit{C} programming language with CPU oriented implementation. However, NCO solvers are usually implemented in the \textit{Python} with GPU oriented parallelizable implementation. Secondly, evaluating speed \textit{between} NCO solvers is also difficult for several reasons. For example, some researches is beneficial to solver single problems fast, the other researches can solve batched problem parallel. Therefore, speed evaluation is just for checking tendency. Note that \textit{AM}, \textit{POMO} and our method have similar neural architecture and solving strategies, they have similar speed to produce solutions.

\textbf{Greedy Rollout Performance.} Continue to the speed evaluation issue, evaluating greedy rollout performance is very meaningful. That is because there are only single chance to produce-validate solution qualities in real-world CO applications such as stochastic CO setting. Some NCO researches improves their performances with \textit{multi-start} sampling scheme which produce multiple solution and select best one. \textit{Multi-start} scheme is beneficial to improves performances using more time-budget but not available for every CO tasks. Note that we also report \textit{multi-start} performance with time-performance analysis. 


\subsection{Tasks and Baselines}

This section provides specific tasks and following baselines. We report our performances in four tasks: TSP, CVRP, PCTSP and OP. 

\textbf{TSP.} TSP is representative problem in COPs, fiding minimum tour-length Hamiltonian cycle. The concorde is state-of-the-art classical solver in TSP. In contructive style NCO models, there are several researches to tackle TSP including PointerNet, S2V-DQN, RL, AM, POMO, MDAM and LCP (only for \textit{multi-start}). There are improvement style NCO models \cite{drl-2opt,ma2021learning}, but we exclude to direct comparison because objective of constructive heurstic and improvement heuristic is different. Note that usually, our method gives better solution in limited time-budget than state-of-the-art deep improvement heuristics, reported in Appendix. Therefore, in this experements, we only report constructive-style DRL-NCO method. 

\textbf{CVRP.} CVRP is variant of TSP where finding minimized tour-length path with limit capacities. When the vehicle exceeded capacities, the vehicle must go back to depot city. Because CVRP is one of the major tasks in operation research (OR) there are several competitive solvers such as hybrid genetic solver (HGS) \cite{vidal2022hybrid}, adaptive large neighborhood search (ALNS) \cite{AZI2014167} and LKH3 \cite{lkh2017}. We only report LKH3 as heuristic baseline because LKH3 is sufficient to outperforms NCO solvers (i.e. LKH3 is still mountain to climb). For (constructive style) DRL-NCO solvers, RL \cite{Nazari}, AM \cite{kool2018attention}, POMO \cite{kwon2020pomo}, MDAM \cite{xin2021multi}  and LCP \cite{kim2021learning}  is reported.

\textbf{PCTSP.} PCTSP is varaint of TSP where fiding minimized tour-length path with prize constraint: vehicle must exceeded prize constraint. Note that vehicle does not have to visit all cities as TSP and CVRP. We follow baseline setting of \cite{kim2021learning} in PCTSP, where iterative local search (ILS) is classical baseline. 

\textbf{OP.} OP is similar with the PCTSP but objective is maximizing total prize and constraint is not exceeding certain tour-length. We follow baseline setting of \cite{xin2021multi} in OP, where \textit{compass} is classical baseline.  

\input{section/5_performance_eval}


%\input{section/5_ablation}

==> section/5_gen_eval.tex <==
\subsection{Scalability Evaluation}





% \begin{table}[t]
% \fontsize{9}{9}\selectfont
% \begin{center}
% \caption{{Performance evaluation results of SymNCO in TSP.\\}}\label{Table01}
% \begin{tabular}{lccccccccc}
% \specialrule{1pt}{0pt}{4pt}
% \multicolumn{1}{l}{\begin{tabular}{c}\multirow{2}{*}{}\end{tabular}}&\multicolumn{3}{c}{Concorde}&\multicolumn{3}{c}{POMO}&\multicolumn{3}{c}{Sym-POMO (\textit{Ours})}\\\cmidrule[0.5pt](lr{0.2em}){2-4} \cmidrule[0.5pt](lr{0.2em}){5-7} \cmidrule[0.5pt](lr{0.2em}){8-10}
% \multicolumn{1}{c}{}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{ Time}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{ Gap}&\multicolumn{1}{c}{Time}
% &\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{Time}\\
% \specialrule{1.0pt}{2pt}{4pt}
% $N=150$  &{15.65}&0.00\%&&\multicolumn{3}{c}{--}&\multicolumn{3}{c}{--}\\
% $N=200$  &{15.65}&0.00\%&&\multicolumn{3}{c}{--}&\multicolumn{3}{c}{--}\\
% $N=500$  &{15.65}&0.00\%&&\multicolumn{3}{c}{--}&\multicolumn{3}{c}{--}\\

% \specialrule{1pt}{1pt}{4pt}

% \end{tabular}
% \end{center}

% \end{table}

\begin{table}[t]
\fontsize{9}{9}\selectfont
\begin{center}
\caption{{Scalability evaluation results of SymNCO in TSP and CVRP.\\}}\label{Table01}
\begin{tabular}{lcccccc}
\specialrule{1pt}{0pt}{4pt}
\multicolumn{1}{l}{\begin{tabular}{c}\multirow{2}{*}{}\end{tabular}}&\multicolumn{3}{c}{TSP ($N=150$)}&\multicolumn{3}{c}{CVRP ($N=150$)}\\\cmidrule[0.5pt](lr{0.2em}){2-4} \cmidrule[0.5pt](lr{0.2em}){5-7}
\multicolumn{1}{c}{}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{ Time}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{ Gap}&\multicolumn{1}{c}{Time}\\
\specialrule{1.0pt}{2pt}{4pt}
LKH3  &&&&&&\\
\cmidrule[1.0pt](lr{0.1em}){1-7}
POMO \{gr.\} &&&&&&\\
POMO (Active Search) &&&&&&\\
\cmidrule[0.7pt](lr{0.1em}){1-7}
Sym-NCO \{gr.\} &&&&&&\\
Sym-NCO (Active Search)  &&&&&&\\
\specialrule{1pt}{1pt}{4pt}


\end{tabular}
\end{center}

\end{table}


==> section/5_performance_eval.tex <==
\subsection{Performance Evaluation}

\textbf{Problem size.} In the main paper, we provide the results of the fixed scale cases $N=100$ and real-world TSP problems TSPLIB of $50<N<250$. 

\textbf{Hyperparameters.} To show \textit{Sym-NCO} can be cope with existing NCO models, we do not change existing NCO model's hyperparameters. For example in TSP and CVRP, we follow same hyperparameters with POMO. We suggested a new hyperparameters; we minimally tuned with certain rules. See appendix for detailed hyperparameters setting and sensitivity. 

\textbf{Dataset and Computing Resources.} We use randomly generated problem for training. We use benchmark dataset (10000 instances) which \cite{kool2018attention} suggested as performance-evaluation. For training and inferences, we use Intel Xeon Scalable Gold CPU and Nvidia A100 single GPU.  



% \begin{table}[t]
% \fontsize{9}{9}\selectfont
% \begin{center}
% \caption{{Performance evaluation results of SymNCO in TSP.\\}}\label{Table01}
% \begin{tabular}{lccccccccc}
% \specialrule{1pt}{0pt}{4pt}
% \multicolumn{1}{l}{\begin{tabular}{c}\multirow{2}{*}{Method}\end{tabular}}&\multicolumn{3}{c}{$N = 20$}&\multicolumn{3}{c}{$N = 50$}&\multicolumn{3}{c}{$N = 100$}\\\cmidrule[0.5pt](lr{0.2em}){2-4} \cmidrule[0.5pt](lr{0.2em}){5-7} \cmidrule[0.5pt](lr{0.2em}){8-10}
% \multicolumn{1}{c}{}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{ Time}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{ Gap}&\multicolumn{1}{c}{Time}
% &\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{Time}\\
% \specialrule{1.0pt}{4pt}{4pt}


 

% Gurobi   &{3.84}&0.00\%&&{5.70}&0.00\%&&{7.76}&0.00\%&\\
% Concorde   &{3.84}&0.00\%&&{5.70}&0.00\%&&{7.76}&0.00\%&\\
% LKH   &{3.84}&0.00\%&&{5.70}&0.00\%&&{7.76}&0.00\%&\\
% OR Tools  &{3.85}&0.37\%&&{5.80}&1.76\%&&8.12&4.53\%& \\
% \cmidrule[1.0pt](lr{0.1em}){1-10}

% {DACT \{$T=1000$\}} &3.84&0.04\%&&5.70&0.14\%&& 7.77&1.62\%& \\
% {DACT \{$T=10000$\}} &3.84&0.00\%&&5.70&0.01\%&& 7.77&0.37\%& \\


% \cmidrule[0.5pt](lr{0.1em}){1-10}
% AM \{gr.\}  &3.84&0.08\%&&5.80& 0.52\%&&8.10&4.53\%&\\
% AM \{$1280$\}  &3.84&0.08\%&&5.73& 0.52\%&&7.94&2.26\%&\\
% \cmidrule[0.5pt](lr{0.1em}){1-10}

% MDAM \{gr.,$5$\}  &3.84&0.05\%&&5.73& 0.04\%&&7.93&0.48\%&\\
% MDAM \{$50$,$5$\}  &3.84&0.00\%&&5.70& 0.04\%&&7.79&0.38\%&\\
% \cmidrule[0.5pt](lr{0.1em}){1-10}


% POMO \{gr.\} &3.84&0.12\%& &5.73&0.64\%& &7.84&1.07\%&\\
% POMO \{$100$\} &3.84&0.04\%& &5.70&0.21\%& &7.80&0.46\%&\\
% POMO \{$800$\} &3.84&0.00\%& &5.70&0.03\%& &7.77&0.14\%&\\

% \cmidrule[0.5pt](lr{0.1em}){1-10}
% Sym-NCO  \{gr.\}  &3.84&0.00\%& &&& &&&\\
% Sym-NCO  \{$100$\}&3.84&0.00\%& &&& &&&\\
% Sym-NCO   \{$800$\}&3.84&0.00\%& &&& &&&\\
% \cmidrule[0.5pt](lr{0.1em}){1-10}
% Sym-NCO*  \{$100,T=100$\}&\textbf{3.84}&0.00\%& &&& &&&\\
% \specialrule{1pt}{0pt}{4pt}

% \end{tabular}
% \end{center}

% \end{table}



% \begin{table}[t]
% \fontsize{8}{8}\selectfont
% \begin{center}
% \caption{{Performance evaluation results of SymNCO.\\}}\label{Table01}
% \begin{tabular}{lcccccccc}
% \specialrule{1pt}{0pt}{4pt}
% \multicolumn{1}{l}{\begin{tabular}{c}\multirow{2}{*}{Method}\end{tabular}}&\multicolumn{2}{c}{TSP ($N = 100$) }&\multicolumn{2}{c}{CVRP ($N = 100$) }&\multicolumn{2}{c}{PCTSP ($N = 100$) }&\multicolumn{2}{c}{OP ($N = 100$) }\\\cmidrule[0.5pt](lr{0.2em}){2-3} \cmidrule[0.5pt](lr{0.2em}){4-5} \cmidrule[0.5pt](lr{0.2em}){6-7}\cmidrule[0.5pt](lr{0.2em}){8-9}
% \multicolumn{1}{c}{}&\multicolumn{1}{c}{Cost $\downarrow$}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{Cost $\downarrow$}&\multicolumn{1}{c}{ Gap}
% &\multicolumn{1}{c}{Cost $\downarrow$}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{Obj.  $\uparrow$}&\multicolumn{1}{c}{Gap}\\
% \specialrule{1.0pt}{2pt}{4pt}

% Concorde   &{7.76}&0.00\% &\multicolumn{2}{c}{--}&\multicolumn{2}{c}{--}&\multicolumn{2}{c}{--}\\
% LKH   &{7.76}&0.00\% &{15.65}&0.00\%&\multicolumn{2}{c}{--}&\multicolumn{2}{c}{--}\\

% ILS C++  &\multicolumn{2}{c}{--}&\multicolumn{2}{c}{--}&{5.98}&0.00\%&\multicolumn{2}{c}{--} \\
% Compass &\multicolumn{2}{c}{--}&\multicolumn{2}{c}{--}&\multicolumn{2}{c}{--}&33.19&0.00\% \\
% OR Tools &8.12&4.53\%&17.16&5.41\%&6.07&1.56\%&\multicolumn{2}{c}{\textit{IF} (10s)} \\
% %\cmidrule[1.0pt](lr{0.1em}){1-13}

% %{DACT \{$T=10000$\}} &{}&{}&{}&15.85& 1.12\%&&\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}} \\


% \cmidrule[0.5pt](lr{0.1em}){1-9}
% AM \{gr.\}   &{8.12}&{4.53\%}&16.80&7.34\%&6.25& 4.46\%&31.62&4.75\%\\


% MDAM \{gr.\times 5\}  &{7.93}&{2.19\%}&16.40& 4.86\%&6.17& 3.13\%&32.32& 2.61\%\\

% POMO \{gr.\} &{7.85}&{1.05\%}&16.26&3.88\%
% &\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}}\\


% Sym-NCO  \{gr.\}  &{\textbf{7.84}}&{\textbf{0.95\%}}&\textbf{16.10}& \textbf{2.84\%} && &&\\



% \cmidrule[0.5pt](lr{0.1em}){1-9}

% AM \{s. 1280\}   &{7.94}&{2.26\%}&16.23&3.72\%&6.25& 4.46\%&31.62&4.75\%\\
% %AM \{$1280$\}  &{}&{}&{}&16.23&3.72\%&&6.08& 0.00\%&&32.68&1.55\%&\\
% %\cmidrule[0.5pt](lr{0.1em}){1-9}

% MDAM \{bs. 30\times 5\}  &{7.80}&{0.48\%}&16.03& 2.49\%&6.17& 3.13\%&32.32& 2.61\%\\
% %MDAM \{$50$,$5$\}  &{}&{}&{}&15.99&2.23\%&&6.06& 1.31\%&&32.96&0.69\%&\\
% %\cmidrule[0.5pt](lr{0.1em}){1-9}

% %POMO \{s.\} &{7.80}&{0.49\%}&16.15&3.00\%
% %&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}}\\
% POMO \{s. 100\} &{7.80}&{0.44\%}&15.90&1.64\%
% &\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}}\\

% %\cmidrule[0.5pt](lr{0.1em}){1-9}
% %POMO \{$100$\} &{}&{}&{}&15.83&0.98\%&&\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}}\\
% %POMO \{$800$\} &{}&{}&{}&15.73&0.32\%& &\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}}\\
% %{DACT \{1K\}} &{7.89}&{1.62\%}&16.17&3.18\%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}} \\
% %{DACT \{10K\}} &{7.79}&{0.37\%}&16.17&3.18\%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}} \\
% %\cmidrule[0.5pt](lr{0.1em}){1-9}

% %Sym-NCO  \{s.\}  &{\textbf{7.79}}&{\textbf{0.44\%}}&& && &&\\
% Sym-NCO  \{s. 100\}  &{\textbf{7.79}}&{\textbf{0.39\%}}&{\textbf{15.87}}& {\textbf{1.44\%}}&& &&\\
% %Sym-NCO  \{2K\}  &{\textbf{7.77}}&{\textbf{0.18\%}}&& && &&\\

% %Sym-NCO*  &{}&{}&{}&&&& \multicolumn{3}{c}{--\textit{}} &\multicolumn{3}{c}{--\textit{}}\\
% %Sym-NCO   \{$100$\}&{}&{}&{}&&& &&& &&&\\
% %Sym-NCO   \{$800$\}&{}&{}&{}&&& &&& &&&\\
% %\cmidrule[0.5pt](lr{0.1em}){1-13}

% %Sym-NCO*  \{$100$, $T=100$\}&{}&{}&{}&&&& \multicolumn{3}{c}{--\textit{}} &\multicolumn{3}{c}{--\textit{}}\\
% \specialrule{1pt}{1pt}{4pt}

% \end{tabular}
% \end{center}

% \end{table}



\begin{table}[t]
\fontsize{9}{9}\selectfont
\begin{center}
\caption{{Performance evaluation results of SymNCO for TSP and CVRP.\\}}\label{Table01}
\begin{tabular}{lccccccc}
\specialrule{1pt}{0pt}{4pt}
\multicolumn{2}{c}{\begin{tabular}{c}\multirow{2}{*}{Method}\end{tabular}}&\multicolumn{3}{c}{TSP ($N = 100$) }&\multicolumn{3}{c}{CVRP ($N = 100$) }\\\cmidrule[0.5pt](lr{0.2em}){3-5} \cmidrule[0.5pt](lr{0.2em}){6-8} 
\multicolumn{2}{c}{}&\multicolumn{1}{c}{Cost $\downarrow$}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{Time}&\multicolumn{1}{c}{Cost $\downarrow$}&\multicolumn{1}{c}{ Gap}&\multicolumn{1}{c}{Time}\\
\specialrule{1.0pt}{2pt}{4pt}


\multicolumn{8}{l}{\textit{Handcrafted Heuristic-based Classical Methods}}\\
\cmidrule[0.5pt](lr{0.1em}){1-8}
Concorde&{Heuristic \cite{concorde}}&{7.76}&0.00\%&{3m}&\multicolumn{3}{c}{--}\\
LKH3&{Heuristic \cite{lkh2017} }   &{7.76}&0.00\%&{21m} &{15.65}&0.00\%&{13h}\\
%OR Tools &8.12&4.53\%&{--}&17.16&5.41\%&{--} \\
%\cmidrule[1.0pt](lr{0.1em}){1-13}

%{DACT \{$T=10000$\}} &{}&{}&{}&15.85& 1.12\%&&\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}} \\


\cmidrule[0.5pt](lr{0.1em}){1-8}

\multicolumn{8}{l}{\textit{RL-based Deep Constructive Heuristic methods with greedy rollout (zero-shot inference)}}\\

\cmidrule[0.5pt](lr{0.1em}){1-8}
PointerNet \{gr.\} &{NIPS'14 \cite{pointer}} & 8.30 & 6.90\% & {--} & \multicolumn{3}{c}{--}\\

S2V-DQN \{gr.\} &{NeurIPS'17 \cite{khalil}} & 8.31 & 7.03\% & {--} & \multicolumn{3}{c}{--}\\

RL \{gr.\} & {NeurIPS'18 \cite{Nazari}} & \multicolumn{3}{c}{--} & 17.23 & 10.12\% & {--}\\

AM \{gr.\}&{ICLR'19 \cite{kool2018attention}}   &{8.12}&{4.53\%}&{6s}&16.80&7.34\%&{8s}\\

POMO \{gr.\}&{NeurIPS'20 \cite{kwon2020pomo}} &{7.85}&{1.05\%}&{6s}&16.26&3.88\%&{8s}\\


MDAM \{gr.\times 5\}&{AAAI'21 \cite{ma2021learning}}  &{7.93}&{2.19\%}&{36s}&16.40& 4.86\%&{45s}\\



\textbf{Sym-NCO}  \{gr.\}&{\textit{This work}}  &{\textbf{7.84}}&{\textbf{0.95\%}}&{6s}&\textbf{16.10}& \textbf{2.84\%}&{8s}\\

\cmidrule[0.5pt](lr{0.1em}){1-8}

\multicolumn{8}{l}{\textit{RL-based Deep Constructive Heuristic methods with multi-start rollout (Post-processing)}}\\

\cmidrule[0.5pt](lr{0.1em}){1-8}

RL \{bs. 10\} & {NeurIPS'18 \cite{Nazari}} & \multicolumn{3}{c}{--} & 16.96 & 8.39\% & {--}\\

AM \{s. 1280\}&{ICLR'19 \cite{kool2018attention}}   &{7.94}&{2.26\%}&{1h}&16.23&3.72\%&{ 2h}\\
%AM \{$1280$\}  &{}&{}&{}&16.23&3.72\%&&6.08& 0.00\%&&32.68&1.55\%&\\
%\cmidrule[0.5pt](lr{0.1em}){1-9}

POMO \{s. 100\}&{NeurIPS'20 \cite{kwon2020pomo}} &{7.80}&{0.44\%}&{11s}&15.90&1.64\%&{19s}\\


MDAM \{bs. 30\times 5\}&{AAAI'21 \cite{ma2021learning}}  &{7.80}&{0.48\%}&{20m}&16.03& 2.49\%&{1h}\\
%MDAM \{$50$,$5$\}  &{}&{}&{}&15.99&2.23\%&&6.06& 1.31\%&&32.96&0.69\%&\\
%\cmidrule[0.5pt](lr{0.1em}){1-9}

%POMO \{s.\} &{7.80}&{0.49\%}&16.15&3.00\%
%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}}\\

%\cmidrule[0.5pt](lr{0.1em}){1-9}
%POMO \{$100$\} &{}&{}&{}&15.83&0.98\%&&\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}}\\
%POMO \{$800$\} &{}&{}&{}&15.73&0.32\%& &\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}}\\
%{DACT \{1K\}} &{7.89}&{1.62\%}&16.17&3.18\%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}} \\
%{DACT \{10K\}} &{7.79}&{0.37\%}&16.17&3.18\%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}} \\
%\cmidrule[0.5pt](lr{0.1em}){1-9}

%Sym-NCO  \{s.\}  &{\textbf{7.79}}&{\textbf{0.44\%}}&& && &&\\

LCP \{s. 1280, 6580\} &{NeurIPS'21 \cite{kim2021learning}}  &{7.81}&{0.54\%}&{>1h*}&15.98& 2.11\%&{>2h*}\\

\textbf{Sym-NCO}  \{s. 100\}&{\textit{This work}}  &{\textbf{7.79}}&{\textbf{0.39\%}}&{11s}&{\textbf{15.87}}& {\textbf{1.44\%}}&{19s}\\
%Sym-NCO  \{2K\}  &{\textbf{7.77}}&{\textbf{0.18\%}}&& && &&\\

%Sym-NCO*  &{}&{}&{}&&&& \multicolumn{3}{c}{--\textit{}} &\multicolumn{3}{c}{--\textit{}}\\
%Sym-NCO   \{$100$\}&{}&{}&{}&&& &&& &&&\\
%Sym-NCO   \{$800$\}&{}&{}&{}&&& &&& &&&\\
%\cmidrule[0.5pt](lr{0.1em}){1-13}

%Sym-NCO*  \{$100$, $T=100$\}&{}&{}&{}&&&& \multicolumn{3}{c}{--\textit{}} &\multicolumn{3}{c}{--\textit{}}\\
\specialrule{1pt}{1pt}{4pt}

\end{tabular}
\end{center}

\end{table}









\begin{table}[t]
\fontsize{9}{9}\selectfont
\begin{center}
\caption{{Performance evaluation results of SymNCO for PCTSP and OP.\\}}\label{Table01}
\begin{tabular}{lccccccc}
\specialrule{1pt}{0pt}{4pt}
\multicolumn{2}{c}{\begin{tabular}{c}\multirow{2}{*}{Method}\end{tabular}}&\multicolumn{3}{c}{PCTSP ($N = 100$) }&\multicolumn{3}{c}{OP ($N = 100$) }\\\cmidrule[0.5pt](lr{0.2em}){3-5} \cmidrule[0.5pt](lr{0.2em}){6-8} 
\multicolumn{2}{c}{}&\multicolumn{1}{c}{Cost $\downarrow$}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{Time}&\multicolumn{1}{c}{Obj $\uparrow$}&\multicolumn{1}{c}{ Gap}&\multicolumn{1}{c}{Time}\\
\specialrule{1.0pt}{2pt}{4pt}


\multicolumn{8}{l}{\textit{Handcrafted Heuristic-based Classical Methods}}\\
\cmidrule[0.5pt](lr{0.1em}){1-8}
ILS C++  &Heuristic&{5.98}&{}&0.00\%&\multicolumn{3}{c}{--} \\
Compass  &Heuristic \cite{compass}&\multicolumn{3}{c}{--}&33.19&0.00\%&{}& 
%OR Tools &8.12&4.53\%&{--}&17.16&5.41\%&{--} \\
%\cmidrule[1.0pt](lr{0.1em}){1-13}

%{DACT \{$T=10000$\}} &{}&{}&{}&15.85& 1.12\%&&\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}} \\


\cmidrule[0.5pt](lr{0.1em}){1-8}

\multicolumn{8}{l}{\textit{RL-based Deep Constructive Heuristic methods with greedy rollout (zero-shot inference)}}\\

\cmidrule[0.5pt](lr{0.1em}){1-8}


%Tsili \{gr.,\textit{GA}\} &{JORS'84}  & \multicolumn{3}{c}{--} & 25.69 & 22.59\% & 5s\\
AM \{gr.\}&{ICLR'19 \cite{kool2018attention}}   &{6.25}&{4.46\%}&{5s}&31.62&4.75\%&{5s}\\


MDAM \{gr.\times 5\}&{AAAI'21 \cite{ma2021learning}} &{6.17}&{3.13\%}&{34s}&32.32& 2.61\%&{32s}\\



\textbf{Sym-NCO}  \{gr.\}&{\textit{This work}}  &{}&{}&{}&& &\\
 
\cmidrule[0.5pt](lr{0.1em}){1-8}

\multicolumn{8}{l}{\textit{RL-based Deep Constructive Heuristic methods with multi-start rollout (Post-processing)}}\\

\cmidrule[0.5pt](lr{0.1em}){1-8}

%Tsili \{s. 1280,\textit{GA}\} &{JORS'84}  & \multicolumn{3}{c}{--} & 30.52 & 8.05\% & 6m\\
AM \{s. 1280\}&{ICLR'19 \cite{kool2018attention}}   &{6.08}&{1.67\%}&{1h}&32.68&1.55\%&{ 53m}\\
%AM \{$1280$\}  &{}&{}&{}&16.23&3.72\%&&6.08& 0.00\%&&32.68&1.55\%&\\
%\cmidrule[0.5pt](lr{0.1em}){1-9}


MDAM \{bs. 30\times 5\}&{AAAI'21 \cite{ma2021learning}}  &{6.07}&{1.46\%}&{16m}&32.91& 0.84\%&{14m}\\


LCP \{1280\} &{NeurIPS'21 \cite{kim2021learning}}  &{6.04}&{1,00\%}&{>1h*}&\multicolumn{3}{c}{--}\\

%MDAM \{$50$,$5$\}  &{}&{}&{}&15.99&2.23\%&&6.06& 1.31\%&&32.96&0.69\%&\\
%\cmidrule[0.5pt](lr{0.1em}){1-9}

%POMO \{s.\} &{7.80}&{0.49\%}&16.15&3.00\%
%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}}\\

%\cmidrule[0.5pt](lr{0.1em}){1-9}
%POMO \{$100$\} &{}&{}&{}&15.83&0.98\%&&\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}}\\
%POMO \{$800$\} &{}&{}&{}&15.73&0.32\%& &\multicolumn{3}{c}{--\textit{}}&\multicolumn{3}{c}{--\textit{}}\\
%{DACT \{1K\}} &{7.89}&{1.62\%}&16.17&3.18\%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}} \\
%{DACT \{10K\}} &{7.79}&{0.37\%}&16.17&3.18\%&\multicolumn{2}{c}{--\textit{}}&\multicolumn{2}{c}{--\textit{}} \\
%\cmidrule[0.5pt](lr{0.1em}){1-9}

%Sym-NCO  \{s.\}  &{\textbf{7.79}}&{\textbf{0.44\%}}&& && &&\\
\textbf{Sym-NCO}  \{s. 100\}&{\textit{This work}}  &{}&{}&{}&{}& {}&{}\\
%Sym-NCO  \{2K\}  &{\textbf{7.77}}&{\textbf{0.18\%}}&& && &&\\

%Sym-NCO*  &{}&{}&{}&&&& \multicolumn{3}{c}{--\textit{}} &\multicolumn{3}{c}{--\textit{}}\\
%Sym-NCO   \{$100$\}&{}&{}&{}&&& &&& &&&\\
%Sym-NCO   \{$800$\}&{}&{}&{}&&& &&& &&&\\
%\cmidrule[0.5pt](lr{0.1em}){1-13}

%Sym-NCO*  \{$100$, $T=100$\}&{}&{}&{}&&&& \multicolumn{3}{c}{--\textit{}} &\multicolumn{3}{c}{--\textit{}}\\
\specialrule{1pt}{1pt}{4pt}

\end{tabular}
\end{center}

\end{table}













\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         \caption{TSP}
         \label{TSP100}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         \caption{CVRP}
         \label{CVRP100}
     \end{subfigure}
     \hfill
          \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         \caption{PCTSP}
         \label{CVRP100}
     \end{subfigure}
     \hfill
          \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         \caption{OP}
         \label{CVRP100}
     \end{subfigure}
        \caption{Time-performance Analysis ($N=100$)}
\end{figure}




% \begin{table}[h]
% \fontsize{9}{9}\selectfont
% \begin{center}
% \caption{{Scalability evaluation results of SymNCO in TSP and CVRP.\\}}\label{Table01}
% \begin{tabular}{lcccccc}
% \specialrule{1pt}{0pt}{4pt}
% \multicolumn{1}{l}{\begin{tabular}{c}\multirow{2}{*}{}\end{tabular}}&\multicolumn{3}{c}{TSP ($N=150$)}&\multicolumn{3}{c}{CVRP ($N=150$)}\\\cmidrule[0.5pt](lr{0.2em}){2-4} \cmidrule[0.5pt](lr{0.2em}){5-7}
% \multicolumn{1}{c}{}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{Gap}&\multicolumn{1}{c}{ Time}&\multicolumn{1}{c}{Cost}&\multicolumn{1}{c}{ Gap}&\multicolumn{1}{c}{Time}\\
% \specialrule{1.0pt}{2pt}{4pt}
% LKH3  &&&&&&\\
% \cmidrule[1.0pt](lr{0.1em}){1-7}
% POMO \{gr.\} &&&&&&\\
% POMO (Active Search) &&&&&&\\
% \cmidrule[0.7pt](lr{0.1em}){1-7}
% Sym-NCO \{gr.\} &&&&&&\\
% Sym-NCO (Active Search)  &&&&&&\\
% \specialrule{1pt}{1pt}{4pt}


% \end{tabular}
% \end{center}

% \end{table}


\textbf{Results in TSP and CVRP.} As shown in Table 1, our \textit{Sym-NCO} outperforms baseline NCO methods both in greedy rollout tasks and multi-start tasks with fastest speed. Remarkably, the \textit{Sym-NCO} achieved $0.95\%$ optimal gap in TSP ($N=100$) using greedy rollout. The speed of greedy rollout in TSP ($N=100$), solving 10000 instances requires only a few second.  

\textbf{Results in PCTSP and OP.} As shown in Table 2, the \textit{Sym-NCO} outperforms every baselines of NCO both in greedy and multi-start tasks. Using multi-start scheme, the \textit{Sym-NCO} can outperforms classical baseline with faster speed. 

\textbf{Time-performance Analysis for Multi-start Scheme.} Using multi-start scheme can improves model's performance giving more time-budget. Therefore, it is natural to compare pareto-curve manner with time-performance graph. As shown in Figure 1, our method have pareto-curve to compare with other NCO baselines. 
 
% \textbf{Scalability Evaluation.} Using \ndref algorithm, our \textit{Sym-NCO} can solve larger size problem TSP ($N=150$) and CVRP ($N=150$). As shown in Table 3, to compare with LKH3, our method can achieve near-optimal solution. Note that this is not argument that our method \textit{ourperforms} LKH3, but just verifying potential scalability of our method. 

==> section/Reviewer_Defense.tex <==
\begin{itemize}
    
    \item \textbf{[Most Questions]} Why NCO? Existing classical methods looks good! (especially Concorde and LKH3) 
    \item Large Scale (N>100) capability: Usually don't read. presentation is important
    \item TSPLIB application (real world distribution problems): Usually don't read. presentation is important
    \item Task flexibility (only routing style?, only for this problem?): Maybe in discussion. 
    \item Specific reason for excluding baseline
    \item Specific policy for hyperparameter selection
    \item Why REINFORCE (few quesition..)?
    \item Clarification to Choose Model, RL method, Hyperparameters, etc..
    \item Clearance of Technical Novelty
    \item This paper is suitable for OR/INforms rather than ICLR/NEURIPS
    \item The authors do not mention whether they will share their code
    
    
    
    
\end{itemize}
